Low-rank on Graphs plus Temporally Smooth Sparse Decomposition for Anomaly Detection in Spatiotemporal Data

Anomaly detection in spatiotemporal data is a challenging problem encountered in a variety of applications including hyperspectral imaging, video surveillance, and urban traffic monitoring. Existing anomaly detection methods are most suited for point anomalies in sequence data and cannot deal with temporal and spatial dependencies that arise in spatiotemporal data. In recent years, tensor-based methods have been proposed for anomaly detection to address this problem. These methods rely on conventional tensor decomposition models, not taking the structure of the anomalies into account, and are supervised or semi-supervised. We introduce an unsupervised tensor-based anomaly detection method that takes the sparse and temporally continuous nature of anomalies into account. In particular, the anomaly detection problem is formulated as a robust lowrank + sparse tensor decomposition with a regularization term that minimizes the temporal variation of the sparse part, so that the extracted anomalies are temporally persistent. We also approximate rank minimization with graph total variation minimization to reduce the complexity of the optimization algorithm. The resulting optimization problem is convex, scalable, and is shown to be robust against missing data and noise. The proposed framework is evaluated on both synthetic and real spatiotemporal urban traffic data and compared with baseline methods.

==> experiments_gloss.tex <==
\section{Experiments}
\label{sec:Exp}

In this paper we evaluated the proposed method on both real and synthetic datasets. To evaluate the effectiveness of the proposed objective function in equation \eqref{eq:aug_lagr}, we compared our method to regular HoRPCA and weighted HoRPCA (WHoRPCA) where the nuclear norm of each unfolding is weighted. To evaluate the effectiveness of the graph regularization, we compared with Low Rank Plus Temporally Smooth Sparse Decomposition (LOSS) corresponding to the objective function given in \eqref{eq:opt_lrt}. As our method is focused on feature extraction for anomaly detection, we also compared our method to baseline anomaly detection methods such as LOF, OCSVM and EE applied to the unprocessed data. After feature extraction stage, unless noted otherwise, such as GLOSS-LOF, EE was used as the default method for computing anomaly scores to compare different approaches. The methods used for comparison and their properties are summarized in Table \ref{tab:methods}.

\begin{table}[]
    \centering
    \caption{Anomaly Detection Methods Compared in the Experiments}
    \begin{tabular}{l c c c c c}
    \toprule
         & L. R. & Sp & Wtd. L. R. & Temp Smooth & Graph R. \\
         \midrule
         GLOSS & + & + &+ &+&+\\
         LOSS & + & + & + & +&- \\
         WHoRPCA & + & + & + &-&-\\
         HoRPCA & + & + & - & - & - \\
         EE & N.A.& N.A.& N.A.& N.A.& N.A. \\
         LOF & N.A.& N.A.& N.A.& N.A.& N.A. \\
         OCSVM & N.A.& N.A.& N.A.& N.A.& N.A. \\
     \bottomrule
    \end{tabular}
    \label{tab:methods}
\end{table}
\subsection{Data and Preprocessing}
To evaluate the proposed framework, we use two publicly available datasets. The first is NYC yellow taxi trip records\footnote{https://www1.nyc.gov/site/tlc/about/tlc-trip-record-data.page} for 2018. This dataset consists of  trip information such as the departure zone and time, arrival zone and time, number of passengers, tips for each yellow taxi trip in NYC. In the following experiments, we only use the arrival zone and time to collect the number of arrivals for each zone aggregated over one hour time intervals. We selected 81 central zones to avoid zones with very low traffic \cite{zhang2019decomposition}. Thus, we created a tensor $\Y$ of size $24\times 7 \times 52 \times 81$ where the first mode corresponds to hours within a day, the second mode corresponds to days of a week, the third mode corresponds to weeks of a year and the last mode corresponds to the zones. %An illustration of the data from an example zone for all Mondays is illustrated in Fig. \ref{fig:nyc_data}. 
The second dataset is Citi Bike NYC bike trips\footnote{https://www.citibikenyc.com/system-data} for 2018. This dataset contains the departure and arrival station numbers, arrival and departure times and user id. In our experiments, we aggregated arrival data for taxi zones imported from the previous dataset to reduce the dimensionality and to avoid data sparsity. Thus, the dimensionality of the data tensor is again $24\times 7 \times 52 \times 81$. 


% \begin{figure}
%     \centering
%     \includegraphics[width=.6\columnwidth]{nyc_mon_times.png}
%     \caption{Arrival data for all Mondays in 2018 for a zone that includes Times Square. }
%     \label{fig:nyc_data}
% \end{figure}
\subsubsection{Synthetic Data generation}

Evaluating urban events in a real-world setting is an open challenge, since it is difficult to obtain urban traffic data sets with ground truth information, i.e. anomalies are not known {\em a priori} and what constitutes an anomaly depends on the nature of the data and the specific problem. To be able to evaluate our method quantitatively, we first generate synthetic data and inject anomalies. Following \cite{zhang2019decomposition}, we generated a synthetic dataset by taking the average of the NYC taxi traffic tensor, $\Y$, along the third mode, i.e. across weeks of a year. We then repeat the resulting three-mode tensor such that for each zone, average data for a week is repeated 52 times, i.e. a years worth of data tensor with dimensionality $24\times7\times52\times81$ is generated. We multiply the tensor entries by white Gaussian noise with $0.3$ to create variation across weeks. We then inject anomalies to the data in randomly selected time intervals during a day by adding or subtracting a constant $c$ times the average of the time interval. The reason for such a choice is that there are many zones which have very low traffic throughout the day. Thus, instead of only multiplying by a value, we also add a value dependent on the properties of the specific time interval. In our experiments, we select random patches of length $7$ for $500$ days, randomly selected from $81$ zones. Thus, in total, there are $3500$ anomalous time points for the whole synthetic data. 

\subsection{Parameter Setting}

Since the variance of the data within each mode and the corresponding ranks are closely related, weights of each mode in the definition of nuclear norm, $\psi_i$s,  are selected as the inverse of the trace of covariance matrix of mode-$i$, i.e. $\psi_{i}=\frac{K}{Tr(\Sigma_{Y_{(i)}})}$, where $K$ is selected such that $\min(\psi_i)=1$. Following \cite{goldfarb2014robust}, we set $\lambda=1/\sqrt{\max(I_1,\dots,I_N)}$ for HoRPCA and $\beta_1=1/5 \text{std}(vec(\Y))$, where $vec(\Y)\in\R^{I_1I_2...I_N}$ is the vectorization of $\Y$. The other $\beta$ parameters for all methods are set to be the same as $\beta_1$. The number of neighbors for LOF is selected as $10$ as this is the suggested lower-bound in \cite{zhang2016tensor}. Finally, the outlier fraction of OCSVM is set to $0.1$.

In Fig. \ref{fig:param_gamvslam} we present AUC values for various $\lambda$ and $\gamma$ for GLOSS. It can be seen that while low $\lambda$ parameters always provide the best results, $\gamma$ values are optimized at around $10^-5$. This shows that sparsity penalty sets the sparse tensor to zero after some point and AUC becomes trivial. The parameter $\gamma$, on the other hand, does not set the whole sparse part to zero but sets all the time intervals to the same value and this is somewhat the same as identifying the anomalous days, which is not the aim of our work and increases false positives. Otherwise, the method is not too sensitive to the selection of parameters.
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{param_gamvslam.png}
    \caption{AUC values for various choices of $\lambda$ and $\gamma$.}
    \label{fig:param_gamvslam}
\end{figure}

\subsection{Experiments on Synthetic Data}
\subsubsection{Robustness against noisy data}
We first experiment on the level of $c$ to analyze the robustness of the method against noise. Since low $c$ means amplitudes of anomalies are low, and they might be inseparable from noise. In Fig. \ref{fig:amp} and Table \ref{tab:nyc_auc}, it can be seen that with various $c$, i.e. varying levels of amplitudes for anomalies, our method improves the results of anomaly detection for EE, LOF and OC-SVM.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{roc_0_1.5_0.1.png}
        \caption{}
        \label{fig:amp1}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{roc_0_2_0.1.png}
        \caption{}
        \label{fig:amp2}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{roc_0_2.5_0.1.png}
        \caption{}
        \label{fig:amp3}
    \end{subfigure}
    \caption{ROC curves for various amplitudes of anomalies. Higher amplitude means more separability. $c=$ (a) $1.5$, (b) $2$, (c) $2.5$.}
    \label{fig:amp}
\end{figure*}


\begin{table}
    \centering
    \caption{AUC values for synthetic data.}
    \begin{tabular}{l c c c}
    \toprule
        & $c=1.5$ & $c=2$ & $c=2.5$\\
    \midrule
        EE & $0.70$ & $0.80$ & $0.87$ \\
        LOF & $0.65$ & $0.72$ & $0.76$ \\
        OCSVM & $0.68$ & $0.78$ & $0.84$ \\
        HoRPCA & $0.50$ & $0.50$ & $0.50$ \\
        WHoRPCA & $0.50$ & $0.50$ & $0.50$ \\
        LOSS & $0.70$ & $0.80$ & $0.87$ \\
        GLOSS-EE & $\mathbf{0.82}$ & $\mathbf{0.92}$ & $\mathbf{0.95}$ \\
        GLOSS-LOF & $0.78$ & $0.89$ & $0.93$ \\
        GLOSS-SVM & $0.80$ & $0.90$ & $0.94$ \\
    \bottomrule
    \end{tabular}
    \label{tab:nyc_auc}
\end{table}

\begin{table*}[]
    \centering
    \caption{AUC values for Fig \ref{fig:amp} (top) and Fig \ref{fig:pctg} (bottom).}
    \begin{tabular}{l|cccccccccc}
    \toprule
    & EE & LOF & OCSVM & HoRPCA & WHoRPCA & LOSS & GLOSS-EE & GLOSS-LOF & GLOSS-SVM
    \\ 
    \midrule
    $c=1.5$ & $0.70$ & $0.65$ & $0.68$ & $0.50$  & $0.50$ & $0.70$ & $\mathbf{0.82}$ & $0.78$ & $0.80$ \\
    $c=2$ & $0.80$ & $0.72$ & $0.78$ & $0.50$  & $0.50$ & $0.80$ & $\mathbf{0.92}$ & $0.89$ & $0.90$ \\
    $c=2.5$ & $0.87$ & $0.76$  & $0.84$ & $0.50$ & $0.50$ & $0.87$ & $\mathbf{0.95}$ & $0.93$ & $0.94$\\ 
    \midrule
    $P = 20\%$ & 0.81 & 0.81 & 0.80 & 0.50 & 0.50 & 0.81 & 0.93 & $\mathbf{0.94}$ & 0.90\\ 
    $P = 40\%$ &0.62 & 0.81 & 0.78 & 0.50 & 0.51 & 0.62 & 0.77 & $\mathbf{0.93}$ & 0.88\\ 
    $P = 60\%$ & 0.54 & 0.76 & 0.74 & 0.50 & 0.50 & 0.54 & 0.61 & $\mathbf{0.87}$ & 0.86\\
    \bottomrule
    \end{tabular}
    \label{tab:nyc_auc}
\end{table*}

\subsubsection{Robustness for missing data}
In addition to injecting synthetic anomalies, we also remove varying amount of days at random from the tensor to evaluate the effectiveness of the methods under missing data. After generating the synthetic data, a percentage $P$ of the of mode-1 fibers, is set to zero to simulate missing data, where the number of fibers is equal to the total number of days, i.e. $7\times 52\times81$. The performance of anomaly detection in this case is illustrated in Fig. \ref{fig:pctg}. It can be seen that the proposed method provides the best anomaly detection performance. While LOF seems to be robust against missing data, applying LOF to the features extracted by our method always provides better performance. However, the best performance is provided by GLOSS-SVM.

\begin{figure*}
    \centering
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{roc_20_2.5_0.1.png}
        \caption{}
        \label{fig:miss20}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{roc_40_2.5_0.1.png}
        \caption{}
        \label{fig:miss40}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{roc_60_2.5_0.1.png}
        \caption{}
        \label{fig:miss60}
    \end{subfigure}
    \caption{ROC curves for various percentage of missing data. $P=$ (a) $20\%$, (b) $40\%$, (c) $60\%$.}
    \label{fig:pctg}
\end{figure*}

The proposed method provides better features for anomaly detection compared to using the original data or features from HoRPCA, WHoRPCA or even LOSS. It can be seen that weighted low-rank approach improves the results compared to HoRPCA. This is due to the fact that the data is not necessarily low-rank along each mode, thus focusing on modes with low variance, improves the accuracy. Moreover, temporal smoothness removes false detection by penalizing instantaneous changes in traffic that do not constitute an actual anomaly which improves the results significantly. Finally a comparison between the results of LOSS and GLOSS shows that graph regularization provides better results by extracting non-linear relationships from data.
Thus, detection of synthetic anomalies is easy for EE. In real data, there might be more than one anomaly or non-anomalous points with higher or lower value at the same time interval of the same day for different weeks for a zone. EE is not robust in the presence of many outliers and missing data due to the underlying assumption of Gaussianity.

\subsection{Experiments on Real Data}
To evaluate the performance of the proposed methods on real data, we compiled a list of 20 urban events that took place in the important urban activity centers such as city squares, parks, museums, stadiums and concert halls, during 2018. To detect the activities, top-$K$ percent, with varying K, of the highest amplitude points of the extracted sparse tensor are selected as anomalies and compared against the compiled list of urban events. 
% \begin{figure}
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{gloss-a.png}
%         \caption{}
%         \label{fig:nyc_real}
%     \end{subfigure}
%     \begin{subfigure}[b]{\columnwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{nyc_bike_real.png}
%         \caption{}
%         \label{fig:nyc_bike_real}
%     \end{subfigure}  
%     \caption{Results on NYC (a) Yellow Taxi Data, (b) Citi Bike Data. }
%     \label{fig:nyc_real}
% \end{figure}
Detection performance for all methods is given in Table \ref{tab:nyc_real} and Table \ref{tab:nyc_bike}.
\begin{table}[]
    \centering
    \caption{Results on 2018 NYC Yellow Taxi Data. Columns indicate the percentage of points with top anomaly scores. Values indicate the number of events detected at corresponding percentage.}
    \begin{tabular}{l c c c c c c c c c}
    \toprule
         \% & 0.014 & 0.07 & 0.14 & 0.3 & 0.7 & 1 & 2 & 3\\
         \midrule
         EE  & 0 & 0 & 1 & 5 & 8 & 9 & 15 & 18\\ 
         LOF & 0 & 0 & 0 & 1 & 1 & 2 & 3 & 5\\
         OCSVM & 0 & 0 & 0 & 3 & 9 & 11 & 14 & 16\\
         HoRPCA & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1\\
         WHoRPCA & 3 & 4 & 4 & 4 & 6 & 7 & 9 & 9\\ 
         LOSS & 0 & 0 & 1 & 5 & 11 & 14 & 16 & 19\\ 
         GLOSS-EE & 1 & 6 & 8 & 12 & 16 & 18 & 19 & 20\\ 
         GLOSS-LOF & 1 & 6 & 8 & 14 & 17 & 18 & 19 & 20\\
         GLOSS-SVM & 0 & 2 & 3 & 7 & 13 & 14 & 17 & 19\\ 
    \bottomrule
    \end{tabular}
    \label{tab:nyc_real}
\end{table}
\begin{table}[]
    \centering
    \caption{Results on 2018 NYC Bike Trip Data. Columns indicate the percentage of points with top anomaly scores. Values indicate the number of events detected at corresponding percentage.}
    \begin{tabular}{l c c c c c c c c c}
    \toprule
         \% & 0.3 & 1 & 2 & 3 & 4.2 & 7 & 9.7 & 12.5\\
         \midrule
         EE  & 0 & 0 & 2 & 2 & 2 & 2 & 2 & 3 \\
         LOF  & 1 & 1 & 1 & 1 & 2 & 2 & 3 & 5\\
         OCSVM  & 0 & 0 & 1 & 2 & 2 & 2 & 4 & 5\\ 
         HoRPCA  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\ 
         WHoRPCA  & 2 & 4 & 6 & 6 & 6 & 6 & 6 & 6\\ 
         LOSS & 1 & 2 & 2 & 2 & 9 & 9 & 10 & 14\\
         GLOSS-EE  & 1 & 1 & 3 & 5 & 9 & 13 & 14 & 14\\
         GLOSS-LOF & 1 & 2 & 2 & 3 & 3 & 3 & 3 & 3\\ 
         GLOSS-SVM  & 1 & 2 & 5 & 5 & 7 & 9 & 10 & 13\\ 
    \bottomrule
    \end{tabular}
    \label{tab:nyc_bike}
\end{table}
As can be seen in Fig. \ref{fig:nyc_real}, GLOSS-EE outperforms all other methods for both datasets. It is very crucial to note that applying anomaly detection methods such as EE, OCSVM and LOF after feature extraction by GLOSS always result in an improved performance. This is also true for LOSS as temporal smoothness allows both detection of events at lower $K$ and high precision. WHorPCA does not always improve the results compared to HoRPCA as can be seen in Fig. \ref{fig:nyc_bike_real}. HoRPCA performs the worst in both datasets as the optimization is not tailored for anomaly detection. LOF cannot easily separate the anomalies from normal data in both datasets. EE performs very well on Taxi Data but its performance is significantly reduced in Bike Data as the latter is much more noisy. OCSVM provides similar results with EE. It is important to note that most of the anomalies cannot be detected at a low $K$ because events such as New Year's Eve or July 4th celebrations change the activity pattern in the whole city and constitute most of the anomalies detected at low $K$ values for Taxi Data, while Bike Data is very noisy with a high number of days, or points at which it would be considered anomalous. Also, the proposed method does not get affected by events such as weather as it can model both low traffic and high traffic in its low rank part as long as the pattern is similar. The deviations from the daily pattern, rather than the traffic amplitude is projected to the sparse part, which are scored as anomaly candidates. Thus, our method is able to extract the remaining activities at a fairly low $K$.  The proposed method can detect both low amplitude anomalies and anomalies that tend to repeat across weeks, reasonably well. 

\begin{figure*}
    \centering
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{bike_case.png}
        \caption{}
        \label{fig:case}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{bike_case_spa.png}
        \caption{}
        \label{fig:case_spa}
    \end{subfigure}
    \begin{subfigure}[b]{.32\textwidth}
        \includegraphics[width=.98\columnwidth]{bike_case_lr.png}
        \caption{}
        \label{fig:case_lr}
    \end{subfigure}
    \caption{Comparison of the Bike Data, extracted sparse part and low rank part for July 4th Celebrations at Hudson River banks. (a) Real Data where 52 Wednesday's of 2018 is shown and Independence Day and average traffic is highlighted. (b) Sparse tensor where the curve corresponding to the anomaly is highlighted. (c) Low rank tensor with the curve corresponding to the Independence Day highlighted.}
\end{figure*}
